The metric space of limit laws for $q$-hook formulas

In earlier work, Billey--Konvalinka--Swanson studied the asymptotic distribution of the coefficients of Stanley's $q$-hook length formula, or equivalently the major index on standard tableaux of straight shape and certain skew shapes. We extend those investigations to Stanley's $q$-hook-content formula related to semistandard tableaux and $q$-hook length formulas of Bj\"orner--Wachs related to linear extensions of labeled forests. We show that, while their coefficients are ``generically'' asymptotically normal, there are uncountably many non-normal limit laws. More precisely, we introduce and completely describe the compact closure of the metric space of distributions of these statistics in several regimes. The additional limit distributions involve generalized uniform sum distributions which are topologically parameterized by certain decreasing sequence spaces with bounded $2$-norm. The closure of these distributions in the L\'evy metric gives rise to the space of DUSTPAN distributions. As an application, we completely classify the limiting distributions of the size statistic on plane partitions fitting in a box.

==> density.tex <==

Anyhow, the general \mathcal{S}_{\mathbf{t}} PDF is:

LEMMA: Let \mathbf{t} = \{t_1, \ldots, t_m > 0\}. Then

\mathrm{PDF}(\mathcal{S}_{\mathbf{t}}; x) = \frac{1}{2(m-1)! t_1 \cdots t_m} \sum_{\epsilon_1, \ldots, \epsilon_m \in \{\pm 1\}} \epsilon_1 \cdots \epsilon_m \left(x + \frac{\epsilon_1 t_1 + \cdots + \epsilon_m t_m}{2}\right)^{m-1} \mathrm{sgn}\left(x + \frac{\epsilon_1 t_1 + \cdots + \epsilon_m t_m}{2}\right).

PROOF SKETCH: The m=1 case reduces to

\mathrm{PDF}(\mathcal{U}[-t_1/2, t_1/2]; x) = \frac{1}{2t_1} \left(\mathrm{sgn}\left(\frac{t_1}{2} + x\right) - \mathrm{sgn}\left(-\frac{t_1}{2} + x\right)\right),

which is easily checked. For the general case, it is routine to check that, for all u>0,

x^k \mathrm{sgn}(x) \ast \frac{1}{2} \left(\mathrm{sgn}(u+x) - \mathrm{sgn}(-u+x)\right) = \frac{1}{k+1} \left((u+x)^{m+1} \mathrm{sgn}(u+x) - (-u+x)^{k+1} \mathrm{sgn}(-u+x)\right).

Here \ast denotes convolution. The claim follows by applying the m=1 case and this identity inductively. \Box

REMARK: When t_1 = \cdots = t_m = 1, the above collapses to

\mathrm{PDF}(\mathcal{IH}_m - m/2; x) = \frac{1}{2(m-1)!} \sum_{k=0}^m (-1)^k \binom{m}{k} \left(x + \frac{m-k}{2} - \frac{k}{2}\right)^{m-1} \mathrm{sgn}\left(x + \frac{m-k}{2} - \frac{k}{2}\right)

Hence we recover the well-known formula for the Irwin--Hall distributions' PDF (see e.g. [Johnson--Kotz--Balakrishnan (1994), Continuous Univariate Distributions Vol. 2, 2nd edition, equation (26.48), p. 296]:

\mathrm{PDF}(\mathcal{IH}_m; x) = \frac{1}{2(m-1)!} \sum_{k=0}^m (-1)^k \binom{m}{k} \left(x - k\right)^{m-1} \mathrm{sgn}\left(x - k\right).

REMARK: A similar formula for the CDF of \mathcal{S}_{\mathbf{t}} as a
sum over the vertices of the hypercube is given in [Barrow--Smith
(1979), Spline Notation applied to a Volume Problem]. See [JKB,
p. 298-300] for relevant discussion.

Dustpan: x^k \mathrm{sgn}(x) \ast \frac{1}{\sigma \sqrt{2\pi}} \exp(-x^2/2\sigma^2), wh

